AutoDAN: Generating Stealthy Jailbreak Prompts on Aligned Large Language Models

The aligned Large Language Models (LLMs) are powerful language understanding and decision-making tools that are created through extensive alignment with human feedback. However, these large models remain susceptible to jailbreak attacks, where adversaries manipulate prompts to elicit malicious outputs that should not be given by aligned LLMs. Investigating jailbreak prompts can lead us to delve into the limitations of LLMs and further guide us to secure them. Unfortunately, existing jailbreak techniques suffer from either (1) scalability issues, where attacks heavily rely on manual crafting of prompts, or (2) stealthiness problems, as attacks depend on token-based algorithms to generate prompts that are often semantically meaningless, making them susceptible to detection through basic perplexity testing. In light of these challenges, we intend to answer this question: Can we develop an approach that can automatically generate stealthy jailbreak prompts? In this paper, we introduce AutoDAN, a novel jailbreak attack against aligned LLMs. AutoDAN can automatically generate stealthy jailbreak prompts by the carefully designed hierarchical genetic algorithm. Extensive evaluations demonstrate that AutoDAN not only automates the process while preserving semantic meaningfulness, but also demonstrates superior attack strength in cross-model transferability, and cross-sample universality compared with the baseline. Moreover, we also compare AutoDAN with perplexity-based defense methods and show that AutoDAN can bypass them effectively.

==> Sections/3-Metod-Merge.tex <==
\section{Method}\label{section_method1}
% We start the elucidation of our method from Sec.~\ref{section_method1}. In this paper, t
% The proposed method AutoDAN can be concisely described as a hierarchical genetic algorithm operating within a fine-grained search space initialized by existing manual prompts, such as those from the DAN series. 
% % To comprehensively outline our approach, 
% In this section, we first introduce the threat model and formulation of jailbreak attacks and introduce our method, AutoDAN. 

\subsection{Preliminaries}\label{preliminaries}
\textbf{Threat model.} Jailbreak attacks are closely related to the alignment method of LLMs. The main goal of this type of attack is to disrupt the human-aligned values of LLMs or other constraints imposed by the model developer, compelling them to respond to malicious questions posed by adversaries with correct answers, rather than refusing to answer. 
Consider a set of malicious questions represented as $Q=\{Q_1, Q_2, \ldots, Q_n\}$, the adversaries elaborate these questions with jailbreak prompts denoted as $J=\{J_1, J_2, \ldots, J_n\}$, resulting in a combined input set $T=\{T_{i}=<J_i, Q_i>\}_{i=1, 2, \ldots, n}$. When the input set $T$ is presented to the victim LLM $M$, the model produces a set of responses $R=\{R_1, R_2, \ldots, R_n\}$. The objective of jailbreak attacks is to ensure that the responses in $R$ are predominantly answers closely associated with the malicious questions in $Q$, rather than refusal messages aligned with human values.

\textbf{Formulation.} Intuitively, it is impractical to set a specific target for the response to a single malicious question, as pinpointing an appropriate answer for a given malicious query is challenging and might compromise generalizability to other questions. Consequently, a common solution~\citep{zou2023universal,lapid2023open} is to designate the target response as affirmative, such as answers beginning with ``Sure, here is how to [$Q_i$].'' By anchoring the target response to text with consistent beginnings, it becomes feasible to express the attack loss function used for optimization in terms of conditional probability.

Within this context, given a sequence of tokens $<x_1, x_2, \ldots, x_m>$, the LLM estimates the probability distribution over the vocabulary for the next token $x_{m+1}$ :
% and can continue to generate a sequence of subsequent tokens $x_{m+2}, x_{m+3}, \ldots, x_{m+k}$ for some $k > 0$. Formally, LLM gives prediction based on all previously observed tokens:
\begin{equation}
x_{m+j} \sim P(\cdot | x_1, x_2, \ldots, x_{m+j-1}), \quad \text{for} \quad j = 1, 2, \ldots, k
\end{equation}
The goal of jailbreak attacks is to prompt the model to produce output starting with specific words (e.g. ``\emph{Sure, here is how to [$Q_i$]}''), namely tokens denoted as $<r_{m+1}, r_{m+2}, \ldots, r_{m+k}>$. Given input $T_{i}=<J_i, Q_i>$ with tokens equals to $<t_1, t_2, \ldots, t_m>$, our goal is to optimize the jailbreak prompts $J_i$ to influence the input tokens and thereby maximize the probability:
\begin{equation}\label{equation_likelihood}
P(r_{m+1}, r_{m+2}, \ldots, r_{m+k} | t_1, t_2, \ldots, t_m) = \prod_{j=1}^{k} P(r_{m+j} | t_1, t_2, \ldots, t_m, r_{m+1}, \ldots, r_{m+j})
\end{equation}

\subsection{AutoDAN}
% AutoDAN is a hierarchical genetic algorithm for structured discrete data optimization.It consists of the following components: (1)Population Initialization; (2) Fitness Evaluation; (3) Hierarchical Genetic Algorithm for structured discrete data optimization. 
% \textcircled{1} Initialization: Given a handcrafted prototype jailbreak prompt, we first use this prompt to initialize a population (Sec.~\ref{initialization}). \textcircled{2} Then for each individual in the population, we conduct a fitness evaluation to measure its ability of jailbreaking (see Sec~\ref{fitness}). \textcircled{3} Based on the score calculated from the fitness evaluation, we conduct selection , crossover, and mutation on the population to create a new prompt group for next iteration(see Sec.~\ref{main_population} and Sec.~\ref{sub_population}). \textcircled{4} Once the population meet the termination criteria (see Sec.~\ref{ends}), the algorithm will end and output the corresponding optimal jailbreak prompt.


% We start a comprehensive description of our method AutoDAN from this section. 
As discussed in the introduction, although current jailbreak methods have limitations, when viewed from a different perspective, existing handcrafted methods have offered a valuable starting point, while the automatic method has introduced a valuable score function that guides the optimization of prompts. 
Thus, we utilize handcrafted jailbreak prompts, such as the DAN series, as an initial point for our semantically meaningful jailbreak prompt.
This approach significantly benefits the initialization of our method since it enables the exploration of jailbreak prompts in a space that is more proximate to the potential solution. Once we have an initialized searching space, it becomes appropriate to employ evolutionary algorithms (e.g., genetic algorithm) based on score function, to identify jailbreak prompts that can effectively compromise the victim LLM.


% As discussed in the introduction, current jailbreak methods have the following limitations: 1) Handcrafted methods lack generalizability and automation;  
% % On the other hand, 
% 2) automatic methods that rely on tokens are unable to bypass the perplexity defense. Interestingly, when viewed from a different perspective, existing handcrafted methods have offered a valuable starting point, while the automatic method has introduced a valuable score function that guides the optimization of prompts. Thus, our insight is to utilize handcrafted jailbreak prompts, such as the DAN series, as an initial point for our semantic jailbreak prompt. This approach significantly benefits the initialization of our method since it enables the exploration of jailbreak prompts in a space that is more proximate to the potential solution. Once we have an initialized searching space, it becomes appropriate to employ evolutionary algorithms (e.g., genetic algorithm) based on score function, to identify jailbreak prompts that can effectively compromise the victim LLM.
Thus, our primary objective is to develop a genetic algorithm that utilizes handcrafted prompts as its initialization point and jailbreak attack loss as its scoring function. However, before implementing such a method, we must address three questions: (1) How do we define an initialization space derived from the provided handcrafted prompt? (2) How to design the fitness score to guide the optimization? (3) More importantly, in a discrete representation space of text, how do we formulate effective policies for sample selection, crossover, and mutation?

\subsection{Population Initialization}\label{initialization}
Initialization policy plays a pivotal role in genetic algorithms because it can significantly influence the algorithm's convergence speed and the quality of the final solution. \textit{To answer the first question}, i.e., design an effective initialization policy for AutoDAN, we should bear in mind two key considerations: 1) The prototype handcrafted jailbreak prompt has already demonstrated efficacy in specific scenarios, making it a valuable foundation; thus, it is imperative not to deviate too far from it. 2) Ensuring the diversity of the initial population is crucial, as it prevents premature convergence to sub-optimal solutions and promotes a broader exploration of the solution space. To preserve the basic features of the prototype handcrafted jailbreak prompt while also promoting diversification, we employ LLMs as the agents responsible for revising the prototype prompt, as illustrated in Alg.~\ref{alg_llm_based}. The rationale behind this scheme is that the modifications proposed by LLM can preserve the inherent logical flow and meaning of the original sentences, while simultaneously introducing diversity in word selection and sentence structure.

\subsection{Fitness evaluation.}\label{fitness} To answer the second question,  since the goal of jailbreak attacks can be formulated as Eq.~\ref{equation_likelihood}, we can directly use a function that calculates this likelihood for evaluating the fitness of the individuals in genetic algorithms. Here, we adopt the log-likelihood that was introduced by~\citet{zou2023universal} as the loss function, namely, given a specific jailbreak prompt $J_i$, the loss can be calculated by:
\begin{equation}\label{equation_loss}
\mathcal{L}_{J_i} = - log (P(r_{m+1}, r_{m+2}, \ldots, r_{m+k} | t_1, t_2, \ldots, t_m))
\end{equation}
To align with the classic setting of genetic algorithms that aim to find individuals with higher fitness, we define the fitness score of $J_i$ as $\mathcal{S}_{J_i}=-\mathcal{L}_{J_i}$.

\subsubsection{AutoDAN-GA.} Based on the initialization scheme and fitness evaluation function, we can further use the genetic algorithm to conduct the optimization. The core of the genetic algorithm is to design the crossover and mutation functions. By using a multi-point crossover scheme, we can develop our first version genetic algorithm AutoDAN-GA. We provide the detailed implementation of AutoDAN-GA in Appendix~\ref{apd_autodan_ga} since, here, we hope to discuss how to formulate more effective policies for handling the structural discrete text data, by using its intrinsic characteristics. 

% To handle the structural discrete data, we propose to leverage multi-point sentence exchange, where \chaowei{xxx} as the crossover policy, and the LLM-based diversification in \autoref{alg_llm_based} as the mutation policy. In such a way, we develop our first version genetic algorithm AutoDAN-GA.
% While AutoDAN-GA has exhibited promising results in our evaluations (Sec.~\ref{experiment_ablation}), 
% we believe that an algorithm specifically more tailored to the discrete and structured characteristics of text would be both more effective and efficient. Thus, here, we systemically answer the third question, i.e., how to formulate effective policies in a discrete space like text.

\subsection{Hierarchical Genetic Algorithm for Structured Discrete Data}\label{hga}
\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-1.1cm}
  \centering
  \includegraphics[width=0.38\textwidth]{Figures/GA_vs_HGA.pdf}
  \caption{
  % The average loss curves show that 
  AutoDAN-HGA conducts optimization consistently, but AutoDAN-GA is stuck at a local minimum.}
  \label{fig_ga_vs_hga}
\vspace{-0.42cm}
\end{wrapfigure}

\subsubsection{AutoDAN-HGA.}  A salient characteristic of text data is its hierarchical structure. Specifically, paragraphs in text often exhibit a logical flow among sentences, and within each sentence, word choice dictates its meaning. Consequently, if we restrict the algorithm to paragraph-level crossover for jailbreak prompts, we essentially confine our search to a singular hierarchical level, thereby neglecting a vast search space. To utilize the inherent hierarchy of text data, our method views the jailbreak prompt as a combination of \textbf{paragraph-level population}, i.e., different combination of sentences, while these sentences, in turn, are formed by \textbf{sentence-level population}, for example, different words. During each search iteration, we start by exploring the space of the sentence-level population such as word choices, then integrate the sentence-level population into the paragraph-level population and start our search on the paragraph-level space such as sentence combination. This approach gives rise to a hierarchical genetic algorithm, i.e., AutoDAN-HGA.
As illustrated in Fig.~\ref{fig_ga_vs_hga}, AutoDAN-HGA surpasses AutoDAN-GA in terms of loss convergence. AutoDAN-GA appears to stagnate at a constant loss score,  suggesting that it is stuck in local minima, whereas AutoDAN-HGA continues to explore jailbreak prompts and reduce the loss.

\textbf{Paragraph-level: selection, crossover and mutation}\label{main_population}

Given the population that is initialized by Alg.~\ref{alg_llm_based}, the proposed AutoDAN will first evaluate the fitness score for every individual in the population following Eq.~\ref{equation_loss}. After the fitness evaluation, the next step is to choose the individuals for crossover and mutation. Let's assume that we have a population containing $N$ prompts. Given an elitism rate $\alpha$, we first allow the top $N*\alpha$ prompts with the highest fitness scores to directly proceed to the next iteration without any modification, which ensures the fitness score is consistently dropping. Then, to determine the remaining $N-N*\alpha$ prompts needed in the next iteration, we first use a selection method that chooses the prompt based on its score. Specifically, the selection probability for a prompt $J_i$ is determined using the softmax function:
\begin{equation}\label{equation_softmax}
P_{J_i} =  \frac{e^{S_{J_i}}}{\sum_{j=1}^{N-N*\alpha} e^{S_{J_j}}}
\end{equation}
After the selection process, we will have $N-N*\alpha$ ``parent prompts'' ready for crossover and mutation. Then for each of these prompts, we perform a multi-point crossover at a probability $p_{crossover}$ with another parent prompt. The multi-point crossover\footnote{Since the multi-point crossover is straightforward, we defer the detailed description to Appendix~\ref{apd_autodan_ga}.} scheme can be summarized as exchanging the sentences of two prompts at multiple breakpoints. Subsequently, the prompts after crossover will be conducted a mutation at a probability $p_{mutation}$. We let the LLM-based diversification introduced in Alg.~\ref{alg_llm_based} to also serve as the mutation function due to its ability to preserve the global meaning and introduce diversity. We delineate the aforementioned process in Alg.~\ref{alg_paragraph_level}. For the $N-N*\alpha$ selected data, this function returns $N-N*\alpha$ offsprings. Combining these offsprings with the elite samples that we preserve, we will get $N$ prompts in total for the next iteration.

% \textbf{Sentence-level: momentum word scoring}\label{sub_population}
% \begin{algorithm}[t]
% \caption{Construct Momentum Word Dictionary}\label{alg_momentum_word}
% \begin{algorithmic}[1]
% \Function{consturct\_momentum\_word\_dict}{$word\_dict, individuals, score\_list, K$}
% \State $word\_scores\gets \{\}$
%     \For{each $individual, score$ in $\text{zip}(individuals, score\_list)$}
%         \State $words \gets$ words from $individual$ not in $filtered$ {\color{lightgray}  \quad \# filtered: list}
%         \For{each $word$ in $words$}
%             \State append $score$ to $word\_scores[word]$ {\color{lightgray} \quad \# word\_scores: dictionary}
%         \EndFor
%     \EndFor
%     \For{each $word, scores$ in $word\_scores$}
%         \State $avg\_score \gets \text{average of } scores$
%         \If{$word$ exists in $word\_dict$}
%             \State $word\_dict[word] \gets (word\_dict[word] + avg\_score)/2$ {\color{lightgray}  \quad \# momentum}
%         \Else
%             \State $word\_dict[word] \gets avg\_score$
%         \EndIf
%     \EndFor
%     \State $sorted\_word\_dict \gets$ $word\_dict$ sorted by values in descending order
%     \State \Return top $K$ items of $sorted\_word\_dict$
% \EndFunction
% \end{algorithmic}
% \end{algorithm}


\textbf{Sentence-level: momentum word scoring}\label{sub_population}

At the sentence level, the search space is primarily around the word choices. After scoring each prompt using the fitness score introduced in Eq.~\ref{equation_loss}, we can assign the fitness score to every word present in the corresponding prompt. Since one word can appear in multiple prompts, we set the average score as the final metric to quantify the significance of each word in achieving successful attacks. To further consider the potential instability of the fitness score in the optimization process, we incorporate a momentum-based design into the word scoring, i.e., deciding the final fitness score of a word based on the average number of the score in current iteration and the last iteration. As detailed in Alg.~\ref{alg_momentum_word}, after filtering out some common words and proper nouns (line 4) , we can obtain a word score dictionary (line 6). From this dictionary, we choose the words with top $K$ scores to replace their near-synonym in other prompts, as described in Alg.~\ref{alg_replace_words}.

\textbf{Termination criteria.}\label{ends}
To ensure the effectiveness and efficiency of AutoDAN, we adopt termination criteria combined with a max iteration test and refusal signals test. If the algorithm has exhausted the maximum number of iterations or no keyword in a set list $L_{refuse}$ is detected in the LLM's top $K$ words of its response, AutoDAN will terminate and return the current optimal jailbreak prompt, which has the highest fitness score. Finally, the AutoDAN-HGA can be delineated in Alg.~\ref{alg_hga}.

\begin{algorithm}[t]
\caption{AutoDAN-HGA}\label{alg_hga}
\begin{algorithmic}[1]
\State \textbf{Input} Prototype jailbreak prompt $J_p$, hyper-parameters
\State Initialize population with LLM-based Diversification in Alg.~\ref{alg_llm_based}
\State Evaluate the fitness score of each individual in population following Eq.~\ref{equation_loss}
\For{$iteration$ in paragraph-level Iterations}
        \State Evaluate the fitness score of each individual in population following Eq.~\ref{equation_loss}
        \If{model responses have no word in $L_{refuse}$}
            \State \Return Optimal jailbreak prompt $J_{max}$ with highest fitness score
        \EndIf
        \State Select elite and parent prompts following Eq.\ref{equation_softmax}
        \State Conduct crossover and mutation on parent prompts
        following Alg.~\ref{alg_paragraph_level}
        \For{$iteration$ in sentence-level Iterations}
            \State Evaluate the fitness score of each individual in population following Eq.~\ref{equation_loss}
            \If{model responses have no word in $L_{refuse}$} \textbf{Break}
            \EndIf
            \State Calculate momentum word score by Alg.~\ref{alg_momentum_word}
            \State Update sentences in each prompt by Alg.~\ref{alg_replace_words}
        \EndFor
        \State Evaluate the fitness score of each individual in population following Eq.~\ref{equation_loss}
        \If{model responses have no word in $L_{refuse}$}
            \State \Return Optimal jailbreak prompt $J_{max}$ with highest fitness score
        \EndIf
\EndFor
\State \Return Optimal jailbreak prompt $J_{max}$ with highest fitness score
\end{algorithmic}
\end{algorithm}



==> Sections/Outdated-3-Method-I.tex <==
\section{Method}}\label{section_method1}
% We start the elucidation of our method from Sec.~\ref{section_method1}. In this paper, t
% The proposed method AutoDAN can be concisely described as a hierarchical genetic algorithm operating within a fine-grained search space initialized by existing manual prompts, such as those from the DAN series. 
% % To comprehensively outline our approach, 
In this section, we first introduce the threat model and formulation of jailbreak attacks (Sec.~\ref{preliminaries}), and introduce our method, AutoDAN. 

\subsection{Preliminaries}\label{preliminaries}
\textbf{Threat model.} Jailbreak attacks are closely related to the alignment method of LLMs. The main goal of this type of attack is to disrupt the human-aligned values of LLMs or other constraints imposed by the model developer, compelling them to respond to malicious questions posed by adversaries with correct answers, rather than refusing to answer. Consider a set of malicious questions represented as $Q=\{Q_1, Q_2, \ldots, Q_n\}$, the adversaries elaborate these questions with jailbreak prompts denoted as $J=\{J_1, J_2, \ldots, J_n\}$, resulting in a combined input set $T=\{T_{i}=<J_i, Q_i>\}_{i=1, 2, \ldots, n}$. When the input set $T$ is presented to the victim LLM $M$, the model produces a set of responses $R=\{R_1, R_2, \ldots, R_n\}$. The primary objective of jailbreak attacks is to ensure that the responses in $R$ are predominantly answers closely associated with the malicious questions in $Q$, rather than refusal messages that are aligned with human values.

\textbf{Formulation.} Intuitively, it is impractical to set a specific target for the response to single malicious question, as pinpointing an appropriate answer for a given malicious query is challenging and might compromise generalizability to other questions. Consequently, a common solution~\citep{zou2023universal,lapid2023open} is to designate the target response as affirmative, such as answers beginning with ``Sure, here is how to [$Q_i$]." By anchoring the target response to text with consistent beginnings, it becomes feasible to express the attack loss function used for optimization in terms of conditional probability. Considering a LLM as a marginal probability model, given a sequence of tokens $<x_1, x_2, \ldots, x_m>$, the LLM estimates the probability distribution over the vocabulary for the next token $x_{m+1}$ and can continue to generate a sequence of subsequent tokens $x_{m+2}, x_{m+3}, \ldots, x_{m+k}$ for some $k > 0$. Formally, LLM gives prediction based on all previously observed tokens:
\begin{equation}
x_{m+j} \sim P(\cdot | x_1, x_2, \ldots, x_{m+j-1}), \quad \text{for} \quad j = 1, 2, \ldots, k
\end{equation}

As mentioned above, the goal of jailbreak attacks is to prompt the model to produce output starting with specific words, namely tokens denoted as $<r_{m+1}, r_{m+2}, \ldots, r_{m+k}>$. Given input $T_{i}=<J_i, Q_i>$ with tokens equals to $<t_1, t_2, \ldots, t_m>$, our goal is to optimize the jailbreak prompts $J_i$ to influence the input tokens and thereby maximize the probability:
\begin{equation}
P(r_{m+1}, r_{m+2}, \ldots, r_{m+k} | t_1, t_2, \ldots, t_m) = \prod_{j=1}^{k} P(r_{m+j} | t_1, t_2, \ldots, t_m, r_{m+1}, \ldots, r_{m+j})
\end{equation}\label{equation_likelihood}

\subsection{AutoDAN}
% AutoDAN is a e include population initialization (Sec. ~\ref{initialization}), fitness evaluation (Sec.~\ref{fitness}), main population (Sec.~\ref{main_population}) and child population (Sec.~\ref{sub_population}) along with their corresponding crossover and mutation policies, and termination criteria (Sec.~\ref{ends}). We also provide background knowledge about the genetic algorithm and hierarchical genetic algorithm in Appendix~\ref{apd_ga}.
\chaowei{Add an overview.}

\subsection{Initializing AutoDAN}\label{initialization}
% We start a comprehensive description of our method AutoDAN from this section. 
As discussed in Sec.~\ref{section_into}, current jailbreak methods have the following limitations: 1) Handcrafted methods lack generalizability and automation;  
% On the other hand, 
2) automatic methods that rely on tokens are unable to bypass the perplexity defense. Interestingly, when viewed from a different perspective, existing handcrafted methods have offered a valuable starting point, while the automatic method has introduced a valuable score function that guides the optimization of prompts. Thus, our insight is to utilize handcrafted jailbreak prompts, such as the DAN series, as an initial point for our semantic jailbreak prompt. This approach significantly benefits the initialization of our method since it enables the exploration of jailbreak prompts in a space that is more proximate to the potential solution. Once we have an initialized searching space, it becomes appropriate to employ evolutionary algorithms (e.g., genetic algorithm) based on score function, to identify jailbreak prompts that can effectively compromise the victim LLM.

Based on the aforementioned analysis, our primary objective is to develop a genetic algorithm that utilizes handcrafted prompts as its initialization point and the jailbreak attack loss as its scoring function. However, before implementing such a method, we must address two questions:
\vspace{-0.15cm}
\begin{itemize}
\item How do we define an initialization space derived from the provided handcrafted prompt?
\vspace{-0.05cm}
\item More importantly, in a discrete space like text, how do we formulate effective policies for sample selection, crossover, and mutation?
\end{itemize}
\vspace{-0.15cm}

\textbf{Population initialization via LLM-based diversification.} Initialization policy plays a pivotal role in genetic algorithms because it can significantly influence the algorithm's convergence speed and the quality of the final solution. \textit{To answer the first question}, i.e., design an effective initialization policy for AutoDAN, we should bear in mind two key considerations: 1) The prototype handcrafted jailbreak prompt has already demonstrated efficacy in specific scenarios, making it a valuable foundation; thus, it is imperative not to deviate too far from it. 2) Ensuring the diversity of the initial population is crucial, as it prevents premature convergence to sub-optimal solutions and promotes a broader exploration of the solution space. To preserve the basic features of the prototype handcrafted jailbreak prompt while also promoting diversification, we employ LLMs as the agent responsible for revising the prototype prompt, as illustrated in Alg.~\ref{alg_llm_based}. The rationale behind this scheme is that the modifications proposed by LLM can preserve the inherent logical flow and meaning of the original sentences, while simultaneously introducing diversity in word selection and sentence structure.
\begin{algorithm}
\caption{LLM-based Diversification}\label{alg_llm_based}
\begin{algorithmic}[1]
\Function{diversification}{$prompt, LLM$}
    \State $\text{message}_{\text{system}}$ $\gets$ ``You are a helpful and creative assistant who writes well."
    \State $\text{message}_{\text{user}}$ $ \gets$ ``Please revise the following sentence with no change to its length and 
    \State \hspace{2.7cm} only output the revised version, the sentence is: $prompt$"
\State \Return $LLM$.get\_response($\text{message}_{\text{system}}, \text{message}_{\text{user}}$)
\EndFunction
\end{algorithmic}
\end{algorithm}

\subsection{Fitness evaluation.}\label{fitness} Since the goal of jailbreak attacks can be formulated as Eq.~\ref{equation_likelihood}, we can directly use a function that calculates this likelihood for evaluating the fitness of the individuals in genetic algorithms. Here, we adopt the log-likelihood that was introduced in~\citep{zou2023universal} as the loss function, namely, given a specific jailbreak prompt $J_i$, the loss can be calculated by:
\begin{equation}
\mathcal{L}_{J_i} = - log (P(r_{m+1}, r_{m+2}, \ldots, r_{m+k} | t_1, t_2, \ldots, t_m))
\end{equation}\label{equation_loss}
To align with the classic setting of genetic algorithms that aim to find individuals with higher fitness, we define the fitness score of $J_i$ as $\mathcal{S}_{J_i}=-\mathcal{L}_{J_i}$.

==> Sections/Outdated-4-Method-II.tex <==
\section{Hierarchical Genetic Algorithm for Structured Discrete Data}\label{section_method2}
\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-1.1cm}
  \centering
  \includegraphics[width=0.38\textwidth]{Figures/GA_vs_HGA.pdf}
  \caption{
  % The average loss curves show that 
  AutoDAN-HGA conducts optimization consistently, but AutoDAN-GA is stuck at a local minimum.}
  \label{fig_ga_vs_hga}
\vspace{-0.42cm}
\end{wrapfigure}

Based on the initialization scheme and fitness evaluation function, we can further leverage multi-point sentences exchange as the crossover policy, and the LLM-based diversification as the mutation policy, to develop a naive genetic algorithm AutoDAN-GA. We provide the detailed implementation of AutoDAN-GA in Appendix~\ref{apd_autodan_ga}. While AutoDAN-GA has exhibited promising results in our evaluations (Sec.~\ref{experiment_ablation}), we believe that an algorithm specifically more tailored to the discrete and structured characteristics of text would be both more effective and efficient. Thus, \textit{from this section, we  systemically answer the second question}, i.e., how to formulate effective policies in a discrete space like text.

A salient characteristic of text data is its hierarchical structure. Specifically, paragraphs in text often exhibit a logical flow among sentences, and within each sentence, word choice dictates its meaning. Consequently, if we restrict the algorithm to paragraph-level crossover for jailbreak prompts, we essentially confine our search to a singular hierarchical level, thereby neglecting a vast search space. To utilize the inherent hierarchy of text data, our method views the jailbreak prompt as a combination of distinct sentences (termed the `main population'), while these sentences, in turn, are formed by specific word choices (termed the `child population'). During each search iteration, we commence by exploring the sub-space of the child population, such as word choices. Subsequently, we integrate the child population into the main population, focusing our search on sentence selection. This approach gives rise to a hierarchical genetic algorithm, i.e., AutoDAN-HGA. As illustrated in Fig.~\ref{fig_ga_vs_hga}, AutoDAN-HGA surpasses AutoDAN-GA in terms of loss convergence. AutoDAN-GA appears to stagnate at a constant loss score,  suggesting it's stuck in local minima, whereas AutoDAN-HGA continues to explore jailbreak prompts and reduce the loss.

\subsection{Paragraph-level: selection, crossover and mutation}\label{main_population}

Given individuals that are initialized by Alg.~\ref{alg_llm_based}, we test the fitness score of every individual following Eq.~\ref{equation_loss}. Considering we have a jailbreak prompt candidate set containing $N$ prompts. Given a elitism rate $\alpha$, we first allow the top $N*\alpha$ prompts with the highest scores to proceed to the next iteration's population. Then, to determine the remaining $N-N*\alpha$ prompts needed in the next iteration's population, we first use a selection method that choose the prompt based on its score. Specifically, the selection probability for a prompt $J_i$ is determined using the softmax function:
\begin{equation}
P_{J_i} =  \frac{e^{S_{J_i}}}{\sum_{j=1}^{N-N*\alpha} e^{S_{J_j}}}
\end{equation}\label{equation_softmax}
After the selection process, we have $N-N*\alpha$ ``parent prompts". Then for each of these prompts, we perform a multi-point crossover at a probability $p_{crossover}$ with another parent prompt. The multi-point crossover\footnote{Since the multi-point crossover is straightforward, we defer the detailed description to Appendix~\ref{apd_autodan_ga}.} scheme exchanges the sentences of two prompts at multiple breakpoints. Furthermore, the prompts after crossover,  termed ``offspring prompts", will experience a mutation at a probability $p_{mutation}$. In our method, the mutation function is also the LLM-based diversification introduced in Alg.~\ref{alg_llm_based}. We delineate the aforementioned process in Alg.~\ref{alg_paragraph_level}. Given the $N-N*\alpha$ selected data, this function returns $N-N*\alpha$ offsprings. When combined with the elite samples that we preserve, we finally get $N$ prompts for the next iteration.

\begin{algorithm}[t]
\caption{Apply Crossover and Mutation}\label{alg_paragraph_level}
\begin{algorithmic}[1]
\Function{apply\_crossover\_and\_mutation}{$selected\_data, *kwargs$}
\State $offsprings\gets []$
    \For{$parent1$, $parent2$ in $selected\_data$ and not yet picked}
        \If{random value $<p_{crossover}$}
            \State $child1, child2 \gets$ \Call{crossover}{$parent1, parent2, num\_points$}
            \State append $child1$ and $child2$ to $offsprings$ {\color{lightgray} \quad \# offsprings: list}
        \Else
            \State append $parent1$ and $parent2$ to $offsprings$
        \EndIf
    \EndFor
    \For{$i$ in Range(Len($offsrpings$))}
        \If{random value $<p_{mutation}$}
            \State $offsrpings[i] \gets$ \Call{diversification}{$offsrpings[i] , LLM$}
        \EndIf
    \EndFor
\State \Return $offsprings$
\EndFunction
\end{algorithmic}
\end{algorithm}

\subsection{Sentence-level: momentum word scoring}\label{sub_population}
\begin{algorithm}[t]
\caption{Construct Momentum Word Dictionary}\label{alg_momentum_word}
\begin{algorithmic}[1]
\Function{consturct\_momentum\_word\_dict}{$word\_dict, individuals, score\_list, K$}
\State $word\_scores\gets \{\}$
    \For{each $individual, score$ in $\text{zip}(individuals, score\_list)$}
        \State $words \gets$ words from $individual$ not in $filtered$ {\color{lightgray}  \quad \# filtered: list}
        \For{each $word$ in $words$}
            \State append $score$ to $word\_scores[word]$ {\color{lightgray} \quad \# word\_scores: dictionary}
        \EndFor
    \EndFor
    \For{each $word, scores$ in $word\_scores$}
        \State $avg\_score \gets \text{average of } scores$
        \If{$word$ exists in $word\_dict$}
            \State $word\_dict[word] \gets (word\_dict[word] + avg\_score)/2$ {\color{lightgray}  \quad \# momentum}
        \Else
            \State $word\_dict[word] \gets avg\_score$
        \EndIf
    \EndFor
    \State $sorted\_word\_dict \gets$ $word\_dict$ sorted by values in descending order
    \State \Return top $K$ items of $sorted\_word\_dict$
\EndFunction
\end{algorithmic}
\end{algorithm}

At the sentence-level, the search space is primarily around the word choices. Having scored each prompt using the fitness score introduced in Eq.~\ref{equation_loss}, we can similarly assign a fitness score to every word present in the prompt. Since one word can appear in multiple prompts, we set the average score as the final metric to quantify the significance of each word in achieving successful attacks. To further consider the potential instability in the optimization process, we incorporate a momentum-based design into the word scoring. As detailed in Alg.~\ref{alg_momentum_word}, after filtering out some common words and proper nouns (line 4) , we can obtain a word score dictionary (line 6). From this dictionary, we choose the words with top $K$ scores to replace their near-synonym in other prompts, as described in Alg.~\ref{alg_replace_words}.

\begin{algorithm}
\caption{Replace Words with Synonyms}\label{alg_replace_words}
\begin{algorithmic}[1]
\Function{replace\_with\_synonym}{$prompt, word\_dict, *kwargs$}
    \For{$word$ in $prompt$}
        \State $synonyms \gets$ find synonym in $word\_dict$
        \State $word\_scores \gets$ scores of $synonyms$ from $word\_dict$
        \For{$synonym$ in $synonyms$}
        \If{random value $<word\_dict[synonym]/\Call{sum}{word\_scores}$}
            \State $prompt \gets prompt$ with  $word$ replaced by $synonym$
            \State \textbf{Break}
        \EndIf
        \EndFor
    \EndFor
    \State \Return $prompt$
\EndFunction
\end{algorithmic}
\end{algorithm}

\subsection{Termination criteria}\label{ends}
To ensure a balance between the effectiveness and efficiency of AutoDAN, we adopt termination criteria combined with a max iteration test and refusal signals test. If the algorithm has exhausted the maximum number of iterations or no keyword in a set list $L_{refuse}$ is detected in the LLM's top $K$ words of its response, AutoDAN will terminate and return the current optimal jailbreak prompt which has highest fitness score. Finally, the AutoDAN-HGA can be delineated in Alg.~\ref{alg_hga}.

\begin{algorithm}[h]
\caption{AutoDAN-HGA}\label{alg_hga}
\begin{algorithmic}[1]
\State \textbf{Input} Prototype jailbreak prompt $J_p$, hyper-parameters
\State Initialize population with LLM-based Diversification in Alg.~\ref{alg_llm_based}
\State Evaluate the fitness score of each individual in population following Eq.~\ref{equation_loss}
\For{$iteration$ in paragraph-level Iterations}
        \State Evaluate the fitness score of each individual in population following Eq.~\ref{equation_loss}
        \If{model responses have no word in $L_{refuse}$}
            \State \Return Optimal jailbreak prompt $J_{max}$ with highest fitness score
        \EndIf
        \State Select elite and parent prompts following Eq.~\ref{equation_softmax}
        \State Conduct crossover and mutation on parent prompts
        following Alg.~\ref{alg_paragraph_level}
        \For{$iteration$ in sentence-level Iterations}
            \State Evaluate the fitness score of each individual in population following Eq.~\ref{equation_loss}
            \If{model responses have no word in $L_{refuse}$} \textbf{Break}
            \EndIf
            \State Calculate momentum word score by Alg.~\ref{alg_momentum_word}
            \State Update sentences in each prompt by Alg.~\ref{alg_replace_words}
        \EndFor
        Evaluate the fitness score of each individual in population following Eq.~\ref{equation_loss}
        \If{model responses have no word in $L_{refuse}$}
            \State \Return Optimal jailbreak prompt $J_{max}$ with highest fitness score
        \EndIf
\EndFor
\State \Return Optimal jailbreak prompt $J_{max}$ with highest fitness score
\end{algorithmic}
\end{algorithm}



==> Templete/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

